Robotic Task Ambiguity Resolution via Natural Language Interaction

Language-conditioned policies have recently gained substantial adoption in robotics as they allow users to specify tasks using natural language, making them highly versatile. While much research has focused on improving the action prediction of language-conditioned policies, reasoning about task descriptions has been largely overlooked. Ambiguous task descriptions often lead to downstream policy failures due to misinterpretation by the robotic agent. To address this challenge, we introduce AmbResVLM, a novel method that grounds language goals in the observed scene and explicitly reasons about task ambiguity. We extensively evaluate its effectiveness in both simulated and real-world domains, demonstrating superior task ambiguity detection and resolution compared to recent state-of-the-art baselines. Finally, real robot experiments show that our model improves the performance of downstream robot policies, increasing the average success rate from 69.6% to 97.1%. We make the data, code, and trained models publicly available at https://ambres.cs.uni-freiburg.de.

==> content/2_related_work_bullets.tex <==
% VLMs
Voxposer {huang2023voxposer}
Manipulate-Anything {duan2024manipulate}

% VLAs
- Octo {octo_2023}: earlier VLA "generalist policy"
- OpenVLA {kim24openvla}: other VLA generalist policy
- Pi-zero {0_black_2024}: VLA trained with flow matching.
- TinyVLA {wen2024tinyvla}: focuses on fast and efficient vla training.

% Planning
- See ECoT related work

% Others
- Embodied Chain-of-Thought{zawalski24ecot}: adds chain of thought reasoning to OpenVLA
- PALO {myers2024policy}: few shot adaptation via task decomposition
- OmniManip {pan2025omnimanip}: uses VLM and (gdino?) to ground task relevant objects like us. but then, they reason about affordances and motion constraints, while we reason about task amb.
- HAMSTER: HIERARCHICAL ACTION MODELS FOR OPEN-WORLD ROBOT MANIPULATION

% Zero shot
- Many works on high-level planning with LLMs (eg code as policies, bohg one with cleaning robot, "Interactive Task Planning with Language Models") (see related work of eCoT)
- Vox poser, etc

% Interaction human-to-robot

%% Classic
- CEILing {chisari2021correct}, 
- survey paper {celemin2022interactive}
- sirius {liu2023robot}
%% Language
- Yell at your robot {shi2024yell}
- AIC MLLM {xiong2024aic} A Feedback Information Extraction module is introduced to recognize the failure cause, allowing AIC MLLM to adaptively correct SE(3) pose predictions for articulated objects.
- RoboReflect: Robotic Reflective Reasoning for Grasping Ambiguous-Condition Objects {luo2025roboreflect} -> enables self-reflection and autonomous error correction in grasping objects with ambiguous affordances

% Interaction robot-to-human

%% Classic
Thrifty Dagger, Fleet Dagger (need to check recent refs of these)
Sirius Fleet has an anomaly detection {liu2024multi}

%% Language
- "Vision-language models as success detectors" {du2023vision}
- "AHA: A Vision-Language-Model for Detecting and Reasoning Over Failures in Robotic Manipulation" {duan2024aha} (many other failure detection works in related work)

% Ambiguity

- "Asking Follow-Up Clarifications to Resolve Ambiguities in Human-Robot Conversation" (2022) {dougan2022asking}. Same task, very different approach -> no vlm, classical object detection
- KnowNo: Robots That Ask For Help!! (2023) {knowno2023} (https://robot-help.github.io/)
- Liang et al (2024a) "Introspective planning: Guiding Language-Enabled Agents to Refine Their Own Uncertainty". (https://introplan.github.io/)

- CLARA: Classifying and Disambiguating User Commands (2024) {park2023clara} (https://clararobot.github.io/)
- "LAP: Using Action Feasibility for Improved Uncertainty Alignment of Large Language Model Planners" (2024) {mullen2024lap} (compares to previous one) (no code available..)



